A Simple Baseline for Travel Time Estimation using Large-Scale Trip Data

The increased availability of large-scale trajectory data around the world provides rich information for the study of urban dynamics. For example, New York City Taxi Limousine Commission regularly releases source-destination information about trips in the taxis they regulate. Taxi data provide information about traffic patterns, and thus enable the study of urban flow -- what will traffic between two locations look like at a certain date and time in the future? Existing big data methods try to outdo each other in terms of complexity and algorithmic sophistication. In the spirit of "big data beats algorithms", we present a very simple baseline which outperforms state-of-the-art approaches, including Bing Maps and Baidu Maps (whose APIs permit large scale experimentation). Such a travel time estimation baseline has several important uses, such as navigation (fast travel time estimates can serve as approximate heuristics for A search variants for path finding) and trip planning (which uses operating hours for popular destinations along with travel time estimates to create an itinerary).

==> 1intro.tex <==
% !TEX root = traveltime.tex
\section{Introduction}
\label{sec:intro}

With the development and popularity of GPS devices, we can obtain an increasing amount of trajectory data from vehicles nowadays. For example, New York City Taxi \& Limousine Commission has made all the taxi trips in 2013 public under the Freedom of Information Law (FOIL)~\cite{nyctaxi}. The dataset contains more than $173$ million taxi trips -- almost half million trips per day. Such big data provide rich information about the city dynamics. Therefore, we ask the question: is it possible to answer some expensive trajectory queries in a more efficient and effective way using such big data?

We approach this question by looking at a fundamental problem -- predicting the travel time between an origin $O$ and a destination $D$. Existing methods employ complex algorithms~\cite{Dean99, KDXZ06, Gonz+07, Yuan+10} or use map services~\cite{googlemap, bingmap} to \emph{first find a shortest/fastest route} between $O$ and $D$, then estimate the travel time for a target route~\cite{RJK13, WZX14}. To achieve good performance, route-based methods are often super-linear in order to deal with the data sparsity issue and to capture the transition time at intersections~\cite{WZX14}. \emph{However, we could potentially avoid finding a route in the first step if we have enough historical trips from $O$ to $D$.}  Note that, even with large-scale data, this is not always possible because of varying traffic conditions at different times and locations. However, if sparsity can be dealt with effectively, these historical trips could provide an accurate estimation without using routes.  For example, if we ask a person how long it takes for him to drive from home to work, the person can immediately answer this question without computing the route first because he has commuted many times between home and work. Similarly, we can take the advantage of big data and estimate the travel time directly by retrieving all the nearby trips between $O$ and $D$. We name such approach as \emph{neighbor-based approach}. This simple approach is obviously \emph{more efficient} because it avoids route computation. We further ask the question: could neighbor-based approach also outperform route-based approach in terms of accuracy?

The route-based approach suffers from several problems. First, the shortest route or fastest route might not be the actual route a person chooses to travel from $O$ to $D$ since the choice of the route is affected by the dynamic traffic condition and personal preference. Second, even if the route is exactly the same route that a user chooses, it remains a tricky task to estimate the travel time for the route. Previous methods~\cite{Pett+98, JCCV01, RiVa04, WaPa05} have used loop detector data which provide travel speed and time of individual road segments. Recent works~\cite{RJK13, WZX14} use trajectories of vehicles (i.e., floating-car data) to better capture the transition time at intersections. However, these methods still suffer from data sparsity problem because they need historical data on individual segments or subpaths of the target route. In addition, it is difficult to fully capture the transitions between segments if only using partial routes. 

On the other hand, our neighbor-based approach implicitly considers different routes between $O$ and $D$ because we do not use actual trajectories. Also, these neighboring trips can better capture all the dynamic transition time at intersections because they cover the complete routes. Therefore, the neighbor-based approach could potentially be more effective than route-based approach. However, simply taking the average of travel time from raw neighboring trips could be problematic for two major reasons. \emph{First, the traffic conditions are very dynamic.} Even if two trips have exactly the same origin and destination, a trip during the peak hour will take much longer time than a trip during the non-peak hour.  The traffic conditions are also affected by seasonality and holidays. Therefore, we need to carefully adjust the travel time based on traffic condition at the starting time of the trip. The challenge lies in how to harness the regularities and irregularities in the traffic condition, and how to take into account the differences of the traffic conditions at different spatial regions. \emph{Second, the real-world data are noisy}. In NYC taxi data, for example, we observe many trips with origin and destination just a few meters away but the reported trip times were several hours. There are also reported trips that are a few minutes long, but travelled more than $100$ miles. If we use all the data without proper filtering of outliers, the estimation could go wrong substantially. The challenge is therefore how to filter those outliers systematically so we only use the good records as neighbors to estimate the travel time.

To solve the challenges above, we propose to consider the traffic conditions using a temporal speed reference learned from the data. We discuss how to use time series model to predict the speed at the current time and how to derive relative speed reference to alleviate the data sparsity issue. In addition, we observe that the speed patterns vary for different region pairs and we propose to further refine the speed reference by considering the spatial regions. To address the data noise issue, we propose a linear regression model by explicitly modeling the distribution of outliers in the data.  And the outliers are automatically detected by fitting the data into the linear model.

We conduct experiments on two large datasets from different countries (NYC in US and Shanghai in China). We evaluate our method using more than $150$ million Manhattan trips. Our method can outperform the baseline methods and also Bing Maps~\cite{bingmap} (even when Bing uses traffic conditions corresponding to the time and the day of week of target trips)\footnote{Google Maps API rate caps prevent proper large-scale comparisons.}. Since NYC taxi data only contain the information on endpoints of the trips (i.e., pickup and drop off locations), to compare our method with route-based method, we use Shanghai taxi data with more than $5$ million trips with complete information of trajectories. On this dataset, our method also significantly outperforms route-based method and Baidu Maps~\cite{baidumap}\footnote{Baidu Maps is more suitable to query trips in China due to restrictions on geographic data in China~\cite{chinaGeoRestrict}.}.


In summary, the contributions of this paper are as follows:
\begin{itemize}
\item We propose to estimate the travel time using neighboring trips from the large-scale historical data.  To the best of our knowledge, this is the first work to estimate travel time without computing the routes.
\item We improve our neighbor-based approach by addressing the dynamics of traffic conditions and by filtering the bad data records.
\item Our experiments are conducted on large-scale real data. We show that our method can outperform state-of-the-art methods as well as online map services (Bing Maps and Baidu Maps).
\end{itemize}

The rest of the paper is organized as follows. Section~\ref{sec:relatedwork} reviews related work. Section~\ref{sec:problem} defines the problem and provides an overview of the proposed approach.  Sections~\ref{sec:neighbor} and~\ref{sec:noise} discuss our method to weight the neighboring trips and our outlier filtering method, respectively. We present our experimental results in Section~\ref{sec:exp} and conclude the paper in Section~\ref{sec:conclusion}. 
